SMAUG: End-to-End Full-Stack Simulation Infrastructure for Deep Learning Workloads

In recent years, there has been tremendous advances in hardware acceleration of deep neural networks. However, most of the research has focused on optimizing accelerator microarchitecture for higher performance and energy efficiency on a per-layer basis. We find that for overall single-batch inference latency, the accelerator may only make up 25-40%, with the rest spent on data movement and in the deep learning software framework. Thus far, it has been very difficult to study end-to-end DNN performance during early stage design (before RTL is available) because there are no existing DNN frameworks that support end-to-end simulation with easy custom hardware accelerator integration. To address this gap in research infrastructure, we present SMAUG, the first DNN framework that is purpose-built for simulation of end-to-end deep learning applications. SMAUG offers researchers a wide range of capabilities for evaluating DNN workloads, from diverse network topologies to easy accelerator modeling and SoC integration. To demonstrate the power and value of SMAUG, we present case studies that show how we can optimize overall performance and energy efficiency for up to 1.8-5x speedup over a baseline system, without changing any part of the accelerator microarchitecture, as well as show how SMAUG can tune an SoC for a camera-powered deep learning pipeline.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}
\fixme{Would it be better if we move the motivation into intro?}
As a motivating example of why overall performance is important, using SMAUG, we profile end-to-end inference 
performance on a range of image classification DNNs and 
break down the overall time spent on accelerator compute, data transfer to/from scratchpads, and 
CPU time spent in the software stack.  We define the term ``accelerator'' in this paper to refer to any independently-programmable
hardware block specialized for a few particular operations.
In this case study, the system uses one NVDLA-inspired DNN accelerator, transfers data over DMA, and 
a single-threaded software stack (see Section \ref{sec:method} for more details). Figure \ref{fig:baseline-cycles} shows that
of the entire execution time,
the time spent waiting on accelerator compute by the accelerator during pure computation only takes up $\sim$25\% on average, 
with the rest of the time taken up by data transfer (34\%) and CPU processing tasks (42\%) like data layout transformations,
tiling, and more. On ResNet50, for example,
CPU processing dominates execution time on the baseline system because of the many expensive tiling operations 
between each of the 50 layers. In some respects, this breakdown is not surprising because the 
performance speedups offered by DNN accelerators can easily make software the primary bottleneck of overall latency.
Nonetheless, this analysis shows several opportunities for optimization that wouldn't have been 
revealed by a layer-by-layer 
analysis, which this paper will explore in more depth. This time breakdown is not unique to SMAUG; similar effects have been observed on industry-grade deep 
learning models written in TensorFlow \cite{emmawang2019}.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth, width=8cm]{plots/baseline_cycles_breakdown.pdf}
\caption{Overall performance on a range of DNNs is bottlenecked by data transfer or CPU processing, because accelerators are so well optimized.}
\vspace{-0.2cm}
\label{fig:baseline-cycles}
% Raw numbers.
% [26.56913711 50.49725944 44.04454548 28.6779213  53.05340646 22.02743057
%  66.30768003 41.59676863]
% [55.18428213 31.01036361 37.97927515 37.71509451 15.86926862 44.56251974
%  18.3177001  34.37692912]
% [18.24658076 18.49237694 17.97617937 33.60698418 31.07732492 33.41004969
%  15.37461988 24.02630225]
\end{figure}

